Reducing Spatial Fitting Error in Distillation of Denoising Diffusion Models

Denoising Diffusion models have exhibited remarkable capabilities in image generation. However, generating high-quality samples requires a large number of iterations. Knowledge distillation for diffusion models is an effective method to address this limitation with a shortened sampling process but causes degraded generative quality. Based on our analysis with bias-variance decomposition and experimental observations, we attribute the degradation to the spatial fitting error occurring in the training of both the teacher and student model. Accordingly, we propose $\textbf{S}$patial $\textbf{F}$itting-$\textbf{E}$rror $\textbf{R}$eduction $\textbf{D}$istillation model ($\textbf{SFERD}$). SFERD utilizes attention guidance from the teacher model and a designed semantic gradient predictor to reduce the student's fitting error. Empirically, our proposed model facilitates high-quality sample generation in a few function evaluations. We achieve an FID of 5.31 on CIFAR-10 and 9.39 on ImageNet 64$\times$64 with only one step, outperforming existing diffusion methods. Our study provides a new perspective on diffusion distillation by highlighting the intrinsic denoising ability of models. Project link: \url{https://github.com/Sainzerjj/SFERD}.

==> figureTexts/cond2.tex <==
\begin{figure}[ht]
    \centering
     \begin{minipage}[t]{0.32\textwidth}
        \centering
    \includegraphics[width=0.95\textwidth]{./figures/delta_x0.pdf}
        \caption{L2 distances of the distillation models with different steps from the ground truth at $t$ on CIFAR10.}
        \label{delta_x0}
    \end{minipage}
    \hspace{.01in}
    \begin{minipage}[t]{0.32\textwidth}
        \centering
    \includegraphics[width=0.96\textwidth]{./figures/cond_loss.pdf}
        \caption{The training loss in noise prediction-based conditional and unconditional diffusion models trained on CIFAR10.}
        \label{cond_loss}
    \end{minipage}
    \hspace{.01in}
    \begin{minipage}[t]{0.30\textwidth}
        \centering
    \includegraphics[width = .96\textwidth]{./figures/cond_delta_x0.pdf}
    \caption{The L2 distances of $\bm {\hat x}_0^t$ of the unconditional and conditional student models with the baseline teacher model at $t$ on CIFAR10.}
    \label{cond_delta_x0}
    \end{minipage}
\end{figure}



==> figureTexts/cond_delta_x0.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width = .8\textwidth]{./figures/cond_delta_x0.pdf}
    \caption{The L2 distances of $\bm {\hat x}_0^t$ between the unconditional and conditional distillation student models with 100 steps and the baseline conditional teacher model (DDIM 1000 steps) at $t$, the bottom left of the figure shows the prediction images of the distillation student models, the first row is unconditional and the second row is conditional.}
    \label{cond_delta_x0}
\end{figure}



==> figureTexts/delta_all.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}[t]{0.47\textwidth}
        \centering
    \includegraphics[width=0.95\textwidth]{./figures/delta_x0.pdf}
        \caption{L2 distances of the unconditional distillation models with different steps from the ground truth images at each sampling stage at the corresponding time points on the CIFAR10.}
        \label{delta_x0}
    \end{minipage}
    \hspace{.05in}
    \begin{minipage}[t]{0.47\textwidth}
        \centering
    \includegraphics[width=0.95\textwidth]{./figures/delta_eps_l2.pdf}
        \caption{Distance between neighboring predicted noises at different sampling steps on the CIFAR10, using the eps-prediction pre-trained model.}
        \label{delta_eps}
    \end{minipage}
\end{figure}


==> figureTexts/delta_eps.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=0.95\textwidth]{./figures/delta_eps_l1.pdf}
        \caption{The visualisation of $||\epsilon_\theta(\bm {\hat x}_t, t)-\epsilon^{truth}||$ using $\epsilon$-prediction pre-trained diffusion model on ImageNet 128$\times$128.}
        \label{delta_eps_l1}
\end{figure}



==> figureTexts/delta_x0.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width = .8\textwidth]{./figures/delta_x0.pdf}
    \caption{L2 distances of the unconditional distillation models with different steps from the ground truth images at each sampling stage at the corresponding time points on the cifar10 dataset}
    \label{delta_x0}
\end{figure}



==> figureTexts/fitting_x0.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width = .8\textwidth]{./figures/fitting_x0.pdf}
    \caption{Left: Predicted $\bm \hat{x}_0^t$ by denoising $\bm x_t$ at time $t$. The first-row use CD, the second-row use CD with the Attention Guidance method and the third-row use MSRD-CD. All models are sampled with 4 steps. Right: Average LPIPS for all time steps.}
    \label{fitting_x0}
\end{figure}

% \begin{figure*}[ht]
%     \centering
%     \begin{subfigure}[b]{0.5\textwidth}
%        \includegraphics[width = .8\textwidth]{./figures/fitting_x0.pdf}
%     \caption{Left: Predicted $\bm \hat{x}_0^t$ by denoising $\bm x_t$ at time $t$. The first-row use CD, the second-row use CD with the Attention Guidance method and the third-row use MSRD-CD. Right: Average LPIPS for all steps.}
%     \label{fitting_x0}
%     \end{subfigure}
%     \hspace{.02in}
%     \begin{subfigure}[b]{0.5\textwidth}
%         \includegraphics[width = .8\textwidth]{}
%         \caption{}\label{}
%     \end{subfigure}%
%     \caption{}
%     \label{}
% \end{figure*}

==> figureTexts/heat_eps.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width = .8\textwidth]{./figures/heat_eps.pdf}
    \caption{}
    \label{heat_eps}
\end{figure}


==> figureTexts/p.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width = .8\textwidth]{./figures/p.pdf}
    \caption{Plot of the time trend of the predicted noise standard deviation and the Pearson correlation coefficient obtained at the decoder corresponding to different resolution layers for the attention mask}
    \label{p}
\end{figure}



==> figureTexts/sigma_blur.tex <==
\figure


==> tableTexts/ablation.tex <==
\begin{table}[t]
\centering
\begin{minipage}[c]{0.5\textwidth}
\centering
\begin{tabular}{c|c|ccc}
\noalign{\smallskip}\noalign{\smallskip}\toprule
$\sigma$ & Baseline& $\sigma=1$ & $\sigma=3$ & $\sigma=5$  \\
\midrule
FID ($\downarrow$)&7.22 & 6.81 & \textbf{6.47} & 6.73 \\
\bottomrule
\end{tabular}
\vspace{5pt}
\caption{\textbf{Ablation study of sigma ($\sigma$) of Gaussian blur.}} \vspace{-10pt}
\label{tab:abl_sigma}
\end{minipage}
\begin{minipage}[c]{0.49\textwidth}
\centering
\begin{tabular}{c|c|ccc}
\noalign{\smallskip}\noalign{\smallskip}\toprule
$\psi$ & Baseline &  $\psi=0.8$ & $\psi=1.0$ & $\psi=1.2$\\
\midrule
FID ($\downarrow$) &7.22 &  6.62  &\textbf{6.47} &  6.79\\
\bottomrule
\end{tabular}
\vspace{5pt}
\caption{\textbf{Ablation study of attention threshold ($\psi$).}} \vspace{-10pt}
\label{tab:abl_masking_thres}
\end{minipage}
\end{table}

==> tableTexts/algorithm_sample.tex <==
% \begin{algorithm}[ht]
%     \centering
%     \caption{Rapid Distillation (RD) Sampling (base)}\label{alg:rd_sampling}
%     \begin{algorithmic}[0]
%         \REQUIRE Trained student model $\bm x_\theta^\mathrm {student}$
%         % \KwSty{Prepare:}{\, pre-trained DPM $\bm{\epsilon}_{\theta}$, trained encoder $\bm{E}_{\varphi}$, trained gradient estimator $\bm{G}_{\psi}$,} \\
%         % \KwIn{sample $\bm{x}$, sampling sequence $\{t_{i}\}_{i=1}^{S}$ where $t_{1}=0$ and $t_{S}=T$}
%         % \KwSty{Run:} \\
%         \STATE$\bm{x}_{T} \sim \mathcal{N}(\bm{0}, \bm{\mathrm{I}})$ 
%         \FOR{$t$ in $T, T-1, ..., 1$}
%         \STATE$\bm{x}_{t-1} = \sqrt{\bar{\alpha}_{t-1}} \bigg(\frac{\bm{x}_{t} - \sqrt{1 - \bar{\alpha}_{t}}{\bm{\epsilon}}_{\theta}(\bm{x}_{t},t)}{\sqrt{\bar{\alpha}_{t}}} \bigg) + \sqrt{1 - \bar{\alpha}_{t-1}} \cdot {\bm{\epsilon}}_{\theta}(\bm{x}_{t},t)$
%         \ENDFOR
%         \RETURN{$\bm{x}_{0}$} 
%     \end{algorithmic}
% \end{algorithm}


\begin{algorithm}[ht]
    \centering
    \caption{SFERD Sampling (original)}\label{alg:sferd_sampling}
    \begin{algorithmic}[0]
        \REQUIRE Trained student model $\bm S_\theta$
        % \KwSty{Prepare:}{\, pre-trained DPM $\bm{\epsilon}_{\theta}$, trained encoder $\bm{E}_{\varphi}$, trained gradient estimator $\bm{G}_{\psi}$,} \\
        % \KwIn{sample $\bm{x}$, sampling sequence $\{t_{i}\}_{i=1}^{S}$ where $t_{1}=0$ and $t_{S}=T$}
        % \KwSty{Run:} \\
        
        \STATE$\bm{x}_{T} \sim \mathcal{N}(\bm{0}, \bm{\mathrm{I}})$ 
        \FOR{$t$ in $T, T-1, ..., 1$}
        \STATE$\bm{x}_{t-1} = \sqrt{\bar{\alpha}_{t-1}} \bigg(\frac{\bm{x}_{t} - \sqrt{1 - \bar{\alpha}_{t}}{\bm{ \epsilon}}_{\theta}(\bm{x}_{t},t)}{\sqrt{\bar{\alpha}_{t}}} \bigg) + \sqrt{1 - \bar{\alpha}_{t-1}} \cdot {\bm{\epsilon}}_{\theta}(\bm{x}_{t},t)$
        \ENDFOR
        \RETURN{$\bm{x}_{0}$} 
    \end{algorithmic}
\end{algorithm}

% \begin{algorithm}[H]
%     \KwSty{Prepare:}{\, pre-trained DPM $\bm{\epsilon}_{\theta}$, trained encoder $\bm{E}_{\varphi}$, trained gradient estimator $\bm{G}_{\psi}$,} \\
%     \KwIn{sample $\bm{x}$, sampling sequence $\{t_{i}\}_{i=1}^{S}$ where $t_{1}=0$ and $t_{S}=T$}
%     \KwSty{Run:} \\
%     $\bm{z} = \bm{E}_{\varphi}(\bm{x})$ \\ 
%     $\bm{x}_{T} \sim \mathcal{N}(\bm{0}, \bm{\mathrm{I}})$ or use inferred $\bm{x}_{T}$ \\
%     \For{$i=S$ \KwTo $2$}{
%         $\hat{\bm{\epsilon}}_{\theta}(\bm{x}_{t_{i}},t_{i}) = \bm{\epsilon}_{\theta}(\bm{x}_{t_{i}},t_{i}) - \sqrt{1 - \bar{\alpha}_{t_{i}}} \cdot \bm{G}_{\psi}(\bm{x}_{t_{i}}, \bm{z}, t_{i})$ \\
%         $\bm{x}_{t_{i-1}} = \sqrt{\bar{\alpha}_{t_{i-1}}} \bigg(\frac{\bm{x}_{t} - \sqrt{1 - \bar{\alpha}_{t_{i}}}\hat{\bm{\epsilon}}_{\theta}(\bm{x}_{t_{i}},t_{i})}{\sqrt{\bar{\alpha}_{t_{i}}}} \bigg) + \sqrt{1 - \bar{\alpha}_{t_{i-1}}} \cdot \hat{\bm{\epsilon}}_{\theta}(\bm{x}_{t_{i}},t_{i})$
%     }
%     \Return{$\bm{x}_{0}$} 
%     \caption{DDIM Sampling(Autoencoding)}
%     \label{algorithm:ddim_sampling}
% \end{algorithm}


==> tableTexts/attn_guidance.tex <==
\begin{table}[ht]
\centering
\small
\begin{tabular}{c|c|ccccccc}
\noalign{\smallskip}\noalign{\smallskip}\toprule
$w$ & baseline & $w=0$ & $w=0.1$ & $w=0.2$ & $w=0.3$ & $w=0.4$ & $w=0.5$\\
\midrule
FID ($\downarrow$) &7.22 & 6.59  & 6.70  &  6.81  & \textbf{6.47} & 6.97 &   6.78   \\
\bottomrule
\end{tabular}
\vspace{5pt}
\caption{\textbf{Ablation study of the attention guidance strength ($\omega$).}} \vspace{-10pt}
\label{tab:guide_attention}
\end{table}


==> tableTexts/attn_threhold.tex <==
% \begin{table}[ht]
% \centering
% \small
% \begin{tabular}{c|ccccc}
% \noalign{\smallskip}\noalign{\smallskip}\toprule
% $\psi$ &  $\psi=0.8$ & $\psi=0.9$ & $\psi=1.0$ & $\psi=1.1$ & $\psi=1.2$\\
% \midrule
% FID ($\downarrow$) &  4.62 & 4.75 &\textbf{4.56} & 4.69& 4.79\\
% IS ($\uparrow$)& 83.60 & 84.35 &\textbf{87.98} &85.72 & 84.54 \\
% \bottomrule
% \end{tabular}
% \vspace{5pt}
% \caption{\textbf{Ablation study of the attention threshold ($\psi$).}} \vspace{-10pt}
% \label{tab:abl_masking_thres}
% \end{table}
\begin{table}[ht]
\centering
\small
\begin{tabular}{c|ccc}
\noalign{\smallskip}\noalign{\smallskip}\toprule
$\psi$ &  $\psi=0.8$ & $\psi=1.0$ & $\psi=1.2$\\
\midrule
FID ($\downarrow$) &  4.62  &\textbf{4.56} &  4.79\\
IS ($\uparrow$)& 83.60  &\textbf{87.98} & 84.54 \\
\bottomrule
\end{tabular}
\vspace{5pt}
\caption{\textbf{Ablation study of the attention threshold ($\psi$).}} \vspace{-10pt}
\label{tab:abl_masking_thres}
\end{table}


==> tableTexts/cond_guidance.tex <==
%\begin{wraptable}{r}{8cm}
% \renewcommand{\arraystretch}{0.9}
% \setlength{\tabcolsep}{3pt} 
\begin{table}[ht]
\centering
\small
\begin{tabular}{lcr}
\noalign{\smallskip}\noalign{\smallskip}\toprule
Model & NFE & FID  \\
\midrule
ADM  &  256  & 6.28  \\
ADM (with attention guidance) & 512  & 5.47 \\
ADM (with CFG) &  512  & 2.91  \\
ADM (with CFG + attention guidance) & 768 & \textbf{2.55}  \\
\bottomrule
\end{tabular}
\vspace{4pt}
\caption{The comparison of classifier-free guidance (CFG) and attention guidance sampling using pre-trained conditional ADM on ImageNet 128$\times$128.}
\label{tab:cond_guidance}
\end{table}



==> tableTexts/main_uncond2.tex <==
% \setlength{\intextsep}{8pt}
% \begin{wraptable}{r}{10cm}
\begin{table*}[ht]
%  \renewcommand{\arraystretch}{1}
% \setlength{\tabcolsep}{2pt} 
\centering
% \footnotesize
\begin{tabular}{lrrrcc}
\noalign{\smallskip}\noalign{\smallskip}\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{NFE} &\multicolumn{2}{c}{CIFAR-10} &{ImageNet 64}& {Bedroom 256} \\
 & & FID ($\downarrow$) & IS ($\uparrow$) &{FID ($\downarrow$)} &{FID ($\downarrow$)} \\
 \midrule
 SFERD-PD & 1 &7.54 $\pm$ 0.03&8.61 $\pm$ 0.02 &14.85 $\pm$ 0.16 \\ 
  SFERD-CD& 1 &\textbf{5.31} $\pm$ 0.01 &\textbf{9.24} $\pm$ 0.03 & \textbf{9.39} $\pm$ 0.03\\ 
 % PD~\cite{salimans2022progressive} & 1 & 14.85 & 7.96 & 19.23   \\
 % CD~\cite{song2023consistency} & 1 & 8.21 & 8.41 & 13.87  \\
%   ViTGAN~\cite{leevitgan} & 1 & 6.66 & 9.3 & \multicolumn{1}{c}{/} \\
% DiffAugment-BigGAN~\cite{zhao2020differentiable} & 1 & 5.61 & 9.16 &  \multicolumn{1}{c}{/}   \\
%     % TransGAN~\cite{jiang2021transgan} & 1 & 9.26 & 9.02 & \multicolumn{1}{c}{/} \\
 \midrule
 SFERD-PD  & 2 & 6.37 $\pm$ 0.03& 8.92 $\pm$ 0.05 &7.53 $\pm$ 0.04 \\
SFERD-CD & 2 &\textbf{4.19} $\pm$ 0.01&\textbf{9.45} $\pm$ 0.02&\textbf{6.08} $\pm$ 0.04 \\
 % PD~\cite{salimans2022progressive} & 2 & 7.64 & 8.85 & 9.71\\
 % CD~\cite{song2023consistency} & 2 & 6.26 & 9.17 & 8.24  \\
  \midrule
 SFERD-PD  & 4 & 3.44 $\pm$ 0.01& 9.32 $\pm$ 0.05 &5.93 $\pm$ 0.08\\
 SFERD-CD  & 4 & \textbf{2.68} $\pm$ 0.02 & \textbf{9.79} $\pm$ 0.03 &\textbf{4.41} $\pm$ 0.02\\
 % PD~\cite{salimans2022progressive} & 4 & 4.28 & 9.25 & 7.22\\
 % CD~\cite{song2023consistency} & 4 & 3.39 & 9.71 & 5.81 \\
  \midrule
 SFERD-EDM & 79 & \textbf{2.04} $\pm$ 0.02 & \textbf{9.91} $\pm$ 0.01 & \textbf{2.47} $\pm$ 0.02\\
 % EDM~\cite{karras2022elucidating} & 79 & 2.35 & 9.82 & 2.99\\
 % DDIM~\cite{song2020denoising} & 128 & 3.96 & 9.51 & 3.71 & 33.16 \\
 SFERD-DDIM  & 1024 & 2.27 $\pm$ 0.12 & 9.80 $\pm$ 0.06 &2.91 $\pm$ 0.05 \\
 % DDIM~\cite{song2020denoising} & 1024 & 2.58 & 9.76 &3.34 \\

\bottomrule
\end{tabular}
\vspace{3pt}
\caption{Sample quality on CIFAR-10 and ImageNet 64$\times$64. SFERD-* represents the implementation of the corresponding model within  SFERD framework. For example, SFERD-PD and SFERD-RD represent the models that refer to ideas of Progressive Distillation (PD) and Consistency Distillation (CD) and imply within SFERD, respectively. Both attention guidance method and semantic encoding-based gradient predictor are introduced.}
\label{tab:i64_cifar10}
\end{table*}
